Federated Active Learning for Target Domain Generalisation

In this paper, we introduce Active Learning framework in Federated Learning for Target Domain Generalisation, harnessing the strength from both learning paradigms. Our framework, FEDALV, composed of Active Learning (AL) and Federated Domain Generalisation (FDG), enables generalisation of an image classification model trained from limited source domain client's data without sharing images to an unseen target domain. To this end, our FDG, FEDA, consists of two optimisation updates during training, one at the client and another at the server level. For the client, the introduced losses aim to reduce feature complexity and condition alignment, while in the server, the regularisation limits free energy biases between source and target obtained by the global model. The remaining component of FEDAL is AL with variable budgets, which queries the server to retrieve and sample the most informative local data for the targeted client. We performed multiple experiments on FDG w/ and w/o AL and compared with both conventional FDG baselines and Federated Active Learning baselines. Our extensive quantitative experiments demonstrate the superiority of our method in accuracy and efficiency compared to the multiple contemporary methods. FEDALV manages to obtain the performance of the full training target accuracy while sampling as little as 5% of the source client's data.

==> sec/1_intro_.tex <==
\section{Introduction}
\label{sec:intro}

\begin{figure}
  \centering
 \includegraphics[trim=0cm 0cm 0cm 0.0cm, clip, width=0.4\textwidth]{images/intro_diagram.png}
  \caption{FEDAL+V High-level framework.}
  \label{fig:fedalv_intro}
\end{figure}
%-------------------------------------------------------------------------
\textcolor{blue}{Notes:  we proposed \emph{FEDALv} to address two important problems in FL: a) the distribution shift among the clients b) the problem with data annotation in each client. Thus our method is equally important to active and federated learning communities.
The existing FL method is blindfolded to the issue of data annotations and assumes that every client has overcome the problem of data annotation. However, in reality, data annotation is a tedious and expensive job. Active learning is a sub-domain in machine learning algorithms dealing with the selection of unlabelled data to query their labels. Most of the past studies are limited to single clients. ....... }

Over the recent years, federated learning (FL) \cite{fed_challenges, fednoniid, moon, fedadg, ffal2019, scaffold, fedavg, fedprox} has re-defined the potential of the data-hungry deep learning models. In this context, we approach the configuration of a centralised server, where a global machine learning model can expand its generalisation from distributed client data. This strategy has attracted development of several applications that can benefit from private-insured data centres or edge devices. Some that integrate FL are found in medical applications like drug discovery \cite{fed_melloddy} or MRI segmentation \cite{fedadg}. Other applications are still running on local edge devices like mobile phones (facial \cite{fedfacerecog} and voice recognition \cite{fedspeech} ) or self-driving vehicles \cite{fedadas}.

With its great capabilities, FL comes with intrinsic challenges \cite{fed_challenges, fed_advances}. One of the main fundamental challenges is the \textit{distribution or domain shift}. This effect usually occurs due to the \emph{data heterogeneity} brought from diverse client domains. There is an assumption in classic machine learning scenarios that available training and test data is iid (independent and identically distributed) \cite{fednoniid}. In FL, predominantly this is not the case, especially when there is little to no knowledge about the local and target domain distribution at the server level.
% Enlist <-> discuss challenges: domain/distribution shift. Assumption that the clients have IID - FDG solution , while domain gen cannot be directly applied. some

In an attempt to overcome the distribution shift challenge, a new area of research has opened as Federated Domain Generalisation (FDG) \cite{liu2021feddg,fedadg,flproto,fedsr,genadj_fldg,fdg_survey}. Generalising on the joint local domains can mitigate these shifts from the target domain. Therefore, standard aggregation techniques like FedAvg \cite{fedavg}, FedProx \cite{fedprox} and SCAFFOLD \cite{scaffold} can be further improved when accounting for the domain generalisation (DG) aspect. On these promising premises, we define the centralised server under the FDG paradigm. We also acknowledge that majority of standard domain generalisation methods \cite{dg_gentounseen, dg_condinvrepr, dg_domainadversarial} are not directly applicable to FL due to privacy concerns.

% FedADG and FedSR
% More recently, FLProto

Despite this, FDG has gained interests with works that find implicit domain-invariant representations at a local client level like FedADG \cite{fedadg} or FedSR \cite{fedsr}. Other attempts propose the DG algorithm at the global level \cite{fedg_genadj} while more holistic solutions derive representations from both client and server models. From some of these combinatorial methods, we identified FCCL \cite{fccl}, which leverages self-supervision and knowledge distillation to obtain FL robust representations. Following similar design, FPL \cite{flproto} proposes protoypes to cluster at local and global side.

Inspired from these works and the benefits of FDG, we introduce \textbf{FEDA} a \textbf{F}ederated Learning pipeline with \textbf{E}nergy-based \textbf{D}omain \textbf{A}lignment. As mentioned before, FEDA follows a centralised server with several data source clients and a tested target client (similar to leave-one-out-domain setting). To solve the generalisation and the target domain alignment, FEDA is comprised of two stages. The first stage happens with the local clients training where two regularisation losses are minimised to promote simple domain-invariant representations. This approach is similar to FedSR in mitigating the distribution shift effect from the global model. The second stage of FEDA is deployed in the server after the aggregation of the local model parameters. Before that, we approximate the local learners as energy-based models (EBMs). Therefore, this allows the global model to generate free-energy in an unsupervised manner \cite{eada}. To adapt the federated model to the target data, we minimise a free-energy alignment loss between the averaged free energies of sources and target. This stage maintains the simple domain-invariant representations by limiting certain source batches to shift from the global representations.

As one of the critical demands of a FL pipeline, \emph{privacy} \cite{fed_challenges} must be assured between the clients. For example, leaking patient sensible information from a hospital would fringe several regulations \cite{liu2021feddg}.
Although in FEDA, the local optimisation stage imposes no risks, the server stage might raise some concerns. Therefore, we introduce a privacy policy after the communications round and aggregation of the global model. The policy guarantees that the global model is passed with active gradients in correspondence of each source and target data while just the predictive classes are kept for the free-energy alignment loss propagation. In this case no data is shared with the server and just the update cycle of the global model's parameters with its losses.

%  introduce motivation of + AL fedalv_intro
The benefits of FL lie in the domain diversity of data that each client builds locally. However, in many scenarios the overall data is 
 not only heterogeneous, but it can be corrupted, unlabelled or just unavailable. Moreover, the local data distribution can be skewed or long-tail. To tackle these possible challenges, we propose \textbf{FEDAL+V} (see Fig. \ref{fig:fedalv_intro}), a Federated Active Learning (FAL) strategy integrated in FEDA for sampling informative data. The selection principle is designed in a way to create the underlying source distribution suitable for the unseen target domain.

% FEDAL+V - selection principle.
A FAL strategy considers an initial pool of labelled data for each client and an unlabelled pool from which to select. Some prior works \cite{ffal2019, fal2022, kafal2023, logo} have considered sampling in a federated manner, but none of them have been applied on different domains or in the context of FDG. Commonly, in FAL, the exploration and exploitation of the data are defined by the number of FL cycles and the budget of client data, respectively. FELDA+V follows a similar approach, however, the fixed overall budget varies from one client to another according to the selection criteria. In designing the selection, we noticed that the global model can increasingly be affected by the distribution shift under limited initial labelled data. Furthermore, in-domain FAL often is sub-optimal when exploring data to unseen domains.

% Evaluations of Feda and Fedalv
FELDA+V firstly overcomes these challenges by following the proposed FDG pipeline, FEDA. Then, once trained with the initial pool of clients data, the free-energy measurements and latent representations are extracted from both target and source unlabelled data. Finally, constricted by the budget, we select the source images that are closer to the top high-energy target samples. The new batches of data are requested to be labelled by the clients for the next FAL cycle. 

To quantify both FEDA and FEDAL+V, we empirically evaluate them on three DG benchmarks: PACS \cite{pacs}, OfficeCaltech \cite{officecaltech} and OfficeHome \cite{officehome}. We show that FEDA achieves state-of-the-art results by a large margin when compared with recent baselines like FedSR or FPL. Moreover, FEDAL+V out-stands both classic AL sampling \cite{Sener2017ActiveApproach, ugcn} and more recent FAL strategies like LoGo \cite{logo}.

% Summary
The contributions can be summarised accordingly:
\begin{itemize}
    \item We introduce FEDA, a new FDG pipeline that proposes to regularise the representation complexity and the free-energies generated between source and target clients.
    \item Following FEDA, we tackle for the first time the FDG with AL data selection. We design FEDAL+V criteria that can leverage informative unlabelled source samples to boost the performance on the unseen (zero-shot) domain.
    \item Through quantitative experiments and visual analysis, we demonstrate the efficacy of the introduced methods over three competitive benchmarks.
\end{itemize}
% Data diversity in FDG, / distributed data collection, client
% data corruption, unlabelled, unavailable.
% To tackle these challenges. FEDAL+V

% Clients usually locally shift from the global model and this creates a bigger issues when we try to find domain invariant representation;
% Related to 2: The domain invariant representations are skewed by clients which depending on the AL stage have little amount of data; making the global model even harder to generalise;

% Domain shift

% \textcolor{green}{Outstanding challenges to the task:
% Data sharing is commonly needed in DG, but imposes risks for FL;
% Clients usually locally shift from the global model and this creates a bigger issues when we try to find domain invariant representation;
% (Related to 2) The domain invariant representations are skewed by clients which depending on the AL stage have little amount of data; making the global model even harder to generalise;
% For AL, computation and complexity of architecture/ DG solutions adds another bottleneck in defining the FAL strategy.
% In-domain AL might not be optimal in DG-AL. How do we aggregate parameters of different clients
% }
% Our proposed scenario stands at the congregation of three research fields: federated learning, domain generalisation and active learning.



